Pseudo-Label Training and Model Inertia in Neural Machine Translation

Like many other machine learning applications, neural machine translation (NMT) benefits from over-parameterized deep neural models. However, these models have been observed to be brittle: NMT model predictions are sensitive to small input changes and can show significant variation across re-training or incremental model updates. This work studies a frequently used method in NMT, pseudo-label training (PLT), which is common to the related techniques of forward-translation (or self-training) and sequence-level knowledge distillation. While the effect of PLT on quality is well-documented, we highlight a lesser-known effect: PLT can enhance a model's stability to model updates and input perturbations, a set of properties we call model inertia. We study inertia effects under different training settings and we identify distribution simplification as a mechanism behind the observed results.

==> limitations.tex <==
\section*{Limitations}
\label{sec:limitation}
Some limitations of our current work are that we focused on relatively high-resourced language pairs and on single-language arc NMT models. Forward-translation is often used in low-resource language arcs in order to augment the relatively scarce amount of parallel training data. An interesting question is how our results apply to low-resource languages, particularly in the scenario where teacher quality is limited and parallel data is potentially of lower quality. Lastly, an interesting question not addressed here is whether the effects can be seen in multilingual models and whether FT augmentation in one language improves quality for other languages.

==> results.tex <==
\section{Results}
\label{sec:results}


==> stability.tex <==

\subsection{Stability}
Unlike the consistency metrics, stability metrics are functions of two models: an original one (e.g. one that is deployed and available to users) and an update of this model which implements an incremental change, presumably to improve quality or other performance aspects. We use the following notation: \textit{A model update} consists of pairs (($\theta_i$, $D_i$, $A_i$), ($\theta_{i+1}$, $D_{i+1}$, $A_{i+1}$), where $\theta_{i}$ and $\theta_{i+1}$ are the parameters of models trained to solve the same task on data sets $D_i$ and $D_{i+1}$. The models themselves may vary in size or architecture, and may be trained using different algorithms $A_i$ and $A_{i+1}$. In practice most such model updates are incremental in one or more dimensions. Throughout this section we test model pairs which keep the model size/architectures intact and vary the random parameter initialization in training, as well as models that vary the training data while keeping everything else identical. 

\subsection{Types of model updates}
\paragraph{Different random initialization} Used in .. \gd{motivation here}, this is the most basic of changes and similar effects can be triggered not just by changing the random generator seed but by any other orthogonal changes, such as hardware changes (references here). 
\paragraph{Data changes} \gd{Maybe drop this, it gets too complicated} In this case we simulate a very common type of model update, which changes the training data to address known issues or to increase it. We test two such types of data changes: 1) the updated model uses 10\% more data, drawn from the same distribution as the original training data and 2) the updated model uses data augmentation to improve gender translation accuracy.

\subsection{Stability and regression metrics}

We define stability is a measure of similarity between outputs, irrespective of quality changes, while regressions measure output changes that result in lower quality. 
\paragraph{\textsc{Stability}} We measure stability as a string similarity between the different outputs and we follow \cite{niu-etal-2020-evaluating} to use a symmetric Bleu-based metric, the harmonic mean between Bleu(Output1, Output2) and Bleu(Output2, Output1). We use Bleu because it is a string-based similarity method using n-gram overlap; we also report exact match percentage (EM), which computes the number of translations that have stayed identical.  
\paragraph{\textsc{nf}} We measure regressions, or \textbf{N}egative \textbf{F}lips in previous work, as the number of sentences for which the quality has degraded relative to the size of the test set. In this paper we use human evaluation to detect regressions: annotators are shown two translations and are asked to rate their quality using a score from 1(worst) to 6(perfect), using 0.2 increments. We use two annotators for each segment, and count as a regression any data point where both annotators find that $\theta_{i+1}$ is worse than $\theta_{i}$, which implies both annotators assessed a gap of at least 0.2 points. We opt for human annotations due to the lack of reliable automatic \textit{segment-level} metrics in MT (citations here). We leave the development of automatic metrics that approximate regressions to future work. 
\paragraph{\textsc{nfi}} Similarly to previous work we measure \textbf{N}egative \textbf{F}lip \textbf{I}mpact as the amount of regressions relative the total errors of $\theta_{i+1}$. We define the total error of a model on a data set as the total gap to the perfect score (summing $6 - score(\theta_{i+1})$ over each data point) while regression errors sum $score(\theta_{i}) - score(\theta_{i+1})$ restricted to cases where $\theta_{i+1}$ is worse than $\theta_{i}$. We compute the score as the average score over the two annotators.   

\gd{Notes:
\begin{itemize}
\item We need to show the measures (differences we show) are relatively robust to annotation variance and noise
\item Task of measuring regressions without direct comparisons, or human evaluations is left to future work. Or maybe we can devise an approximate method to do this without human evals? E.g. on multi-reference test sets.
\end{itemize}
}

\subsection{Results}

We hypothesize that models that are trained using self-training data exhibit less variance in their behaviour, leading to more stable updates. 
Specifically, we keep the update definitions identical (such as random initialization variations), and test three contrastive settings: 
\begin{itemize}
    \item \textbf{Baseline:} $D_i$ and $D_{i+1}$ are training data sets as originally defined in the respective update.
    \item \textbf{DS (Distribution Simplification):} $D_i$ and $D_{i+1}$ both contain forward translation data created with similar but \textit{different} models. This tests the hypothesis that using forward translation data in training leads to more stable models that behave similarly when varying minor training conditions. 
    \item \textbf{Distillation:} $D_{i+1}$ augments $D_i$ using forward translation data obtained with model $\theta_i$. In these experiments we distill the entire train data $D_i$ and merge it with the original $D_i$ to create $D_{i+1}$. This setting is a standard distillation approach for minimizing regressions, where $\theta_{i+1}$ is trained to explicitly mimic $\theta_{i}$. 
\end{itemize}

Results are shown in Table \ref{tab:stability}.

\begin{table}[t]
\centering
\begin{tabular}{l|r|rr}
\toprule
   &           & \multicolumn{2}{c}{Regressions} \\
   \cline{3-4}
Model & Stability & \textsc{nf} & \textsc{nfi}  \\
\hline
Baseline &  58.03 &  & \\
Distillation & 69.43 &  &  \\
FT &  &  &  \\
\gd{FT(WMT)} & 80.23 &   &   \\
\gd{BT(WMT)} & 64.64 & & \\
\bottomrule
\hline
\end{tabular}
\caption{Experiments showing the average stability. We define stability as the harmonic mean of BLEU scores between two different models trained with different initializations.}
\label{tab:stability}
\end{table}

